The rank 2 classification problem I: scale invariant geometries

In this first of a series of three papers we outline an approach to classifying 4d $\mathcal{N}{=}2$ superconformal field theories at rank 2. The classification of allowed scale invariant $\mathcal{N}=2$ Coulomb branch geometries of dimension (or rank) greater than one is a famous open problem whose solution will greatly constrain the space of $\mathcal{N}{=}2$ superconformal field theories. At rank 2 the problem is equivalent to finding all possible genus 2 Seiberg-Witten curves and 1-forms satisfying a special K\"ahler condition. This is tractable because regular genus 2 Riemann surfaces can be uniformly described as binary-sextic plane curves, and the Seiberg-Witten curves are families of such curves varying meromorphically over the two-dimensional base. There are also solutions consisting of families of degenerate genus-2 Riemann surfaces given by a bouquet of two elliptic curves which are described by a different set of curves. In this paper we set up and carry out the analysis of the generic case, i.e., those whose typical fiber is a regular genus-2 Riemann surface with no extended automorphism, and find the complete answer for polynomial coefficients.

==> Tables/Rank-1_theories.tex <==
\begin{table}[tp]
\hspace*{-0.8cm}
\def\arraystretch{1}%
\begin{tabular}{c|c|c|c|c|c|c|c|cc}
Name & \multicolumn{1}{c|}{$12\, c_{\mathrm{4d}}$ } & $\D_u$ &$h_{\mathrm{ECB}}$&$\mathbf{R}$ & $T(\mathbf{R})$& $b$&$\mathfrak{g}$&$ k_{\mathfrak{g}}$  \\
\hhline{=========}
$ \cT^{(1)}_{E_8,1}$ &62&6&0&${\mathbf1}$&0& 10&$\ef_8$&12 
\\
$\cT^{(1)}_{E_7,1}$ &38&4&0&${\mathbf1}$&0&9&$\ef_7$&8\\
 $\cT^{(1)}_{E_6,1} / [\cT^{(1)}_{E_6,1}]_{\ZZ_2}$ &26&3&0&${\mathbf1}$&0&8&$\ef_6/ \mathfrak{f}_4$&6\\
$\cT^{(1)}_{D_4,1}/[\cT^{(1)}_{D_4,1}]_{\ZZ_2}/[\cT^{(1)}_{D_4,1}]_{\ZZ_3}$ &14&2&0&${\mathbf1}$&0&6&$\sof(8)/ \mathfrak{so}(7)/\mathfrak{g}_2$&4\\
$\cT^{(1)}_{A_2,1}/[\cT^{(1)}_{A_2,1}]_{\ZZ_2}/[\cT^{(1)}_{A_2,1}]_{\ZZ_3}$ &8&$\frac32$&0&${\mathbf1}$&0&4&$\suf(3)/\suf(3)/\suf(2)$&3\\
$\cT^{(1)}_{A_1,1}/[\cT^{(1)}_{A_1,1}]_{\ZZ_2}$ &6&$\frac43$&0&${\mathbf1}$&0&3&$\suf(2)/\suf(2)$&$\frac83$\\
 $\cT^{(1)}_{\varnothing,1}$ &$\frac{22}5$&$\frac65$&0&${\mathbf1}$&0&2&$\varnothing$&$\star$\\
\cdashline{1-9}
$\cS^{(1)}_{E_6,2}$&49&6&5&${\mathbf{10}}$&1&7&$\spf(10)$&7&\\
$\cS^{(1)}_{D_4,2}$&29&4&3&$({\mathbf{6,1}})$&1&6&$\spf(6){\times} \suf(2)$&(5,8)&\\
$\cS^{(1)}_{A_2,2}/[\cS^{(1)}_{A_2,2}]_{\ZZ_2}$&19&3&2&${\mathbf4}_0$&1&5&$\spf(4){\times} \uf(1)/ \mathfrak{sp}(4)$&$(4,\star)$\\
$\blue{\cS^{(1)}_{\varnothing,2}}$&9&2&1&${\mathbf2}$&1& 3&$\suf(2)$&3\\
\cdashline{1-9}
$\cS^{(1)}_{D_4,3}$&42&6&4&${\mathbf4}\oplus\bar{\mathbf 4}$&2&6&$\suf(4)$&14\\
$\cS^{(1)}_{A_1,3}$&24&4&3&${\mathbf2}_+\oplus{\mathbf 2}_-$&2&5&$\suf(2){\times}\uf(1)$&$(10,\star)$\\
$\green{\cS^{(1)}_{\varnothing,3}}$&15&3&1&${\mathbf1}_+\oplus{\mathbf 1}_-$&0&4&$\uf(1)$&$\star$ \\
\cdashline{1-9}
$\cS^{(1)}_{A_2,4}$&38&6&3&${\mathbf3}\oplus\bar{\mathbf 3}$&2&$\frac{11}2$&$\suf(3)$&14\\
$\green{\cS^{(1)}_{\varnothing,4}}$&21&4&1&${\mathbf1}_+\oplus{\mathbf 1}_-$&0&$\frac92$&$\uf(1)$&$\star$
\end{tabular}
\caption{\small The list of rank-one SCFTs which can describe the low-energy physics on codimension-one singular loci of the Coulomb branch. Additional information can be found in \cite{Argyres:2016yzz}. Theories in green are $\cN=3$, while the  theory in blue is $\cN=4$.\red{Remove some columns and add a Kodaira type one}
\label{tab:R1Theories}}
\end{table}%
